5 radio sources of the Zenith survey at RATAN-600: VLA maps, radio spectra and optical identification

VLA maps obtained at 1.4 GHz with a resolution of 2\farcs5$\times$2\arcsec for three sources and 6\farcs5$\times$2\farcs3 for two sources detected in the RATAN-600 Zenith survey of 1988 have been analyzed. All five objects have an extended structure. Continuous radio spectra of these objects prepared by using the CATS database and RATAN-600 observations are given. All five objects have linear steep spectra ($\alpha < -0.65$). Using APM database and DSS we have found three candidates for identification. Two radio sources have been observed with the 6 m telescope. The nature of the studied objects, one of which is classified as QSO (BSO) and two others as galaxies, is discussed. One of the radio sources, RZ5, being a merging group of one large and several small galaxies, may have appeared in this process.

==> abstract <==
%auto-ignore
\\
Title: 5 radio sources of the Zenith survey at RATAN-600:
       VLA maps, radio spectra and optical identification
Authors: Yu.N.Parijskij (1), W.M. Goss (2), O.V.Verkhodanov (1),
	 A.I.Kopylov (1), N.S.Soboleva (1), A.V.Temirova (1)
	((1) Special astrophysical observatory, Russia;
	 (2) National Radio Astronomy Observatory, USA)
Comments: 12 pages, 12 figures, uses sao2.sty and psfig.sty
Report-no:
Subj-class:  Astrophysics
Journal-ref: Bulletin of SAO, 1999, No 48, PP.5-16, in press
\\
VLA maps obtained at 1.4 GHz
with a resolution of 2\farcs5$\times$2\arcsec~for three sources and
6\farcs5$\times$2\farcs3 for two sources
detected  in the RATAN--600 Zenith survey of 1988
have been analyzed. All five objects have an extended structure.
Continuous radio spectra of these objects prepared by using
the CATS database and RATAN-600 observations are given.
All five objects have linear steep spectra ($\alpha < -0.65$).
Using APM database and DSS we have found three candidates for identification.
Two radio sources have been observed with the 6 m telescope.
The nature of the studied objects, one of which is classified as QSO (BSO)
and two others as galaxies, is discussed.
One of the radio sources, $RZ5$, being a merging group of one large and
several small galaxies, may have appeared in this process.
\\

